Cold diffuse interstellar medium of Magellanic Clouds: II. Physical conditions from excitation of CI and H$_2$

We present a comprehensive study of the excitation of CI fine-structure levels along 57 sight lines in the Large and Small Magellanic Clouds. The sight lines were selected by the detection of H$_2$ in FUSE spectra. Using archival HST/COS and HST/STIS spectra we detected absorption of CI fine-structure levels and measured their populations for 29 and 22 sight lines in the LMC and SMC, respectively. The CI column density ranges from $10^{13}$ to $10^{14}\,{\rm cm}^{-2}$ for the LMC and $10^{13}$ to $10^{15.4}\,{\rm cm}^{-2}$ for the SMC. We found excitation of CI fine-structure levels in the LMC and SMC to be 2-3 times higher than typical values in local diffuse ISM. Comparing excitation of both CI fine-structure levels and H$_2$ rotational levels with a grid of PDR Meudon models we find that neutral cold gas in the LMC and SMC is illuminated by stronger UV field than in local ISM ($\chi=5^{+7}_{-3}$ units of Mathis field for the LMC and $2^{+4}_{-1}$ for the SMC) and has on average higher thermal pressure ($\log p/k =4.2\pm0.4$ and $4.3\pm0.5$, respectively). Magellanic Clouds sight lines likely probe region near star-formation sites, which also affects the thermal state and CI/H$_2$ relative abundances. At the same time such high measurements of UV field are consistent with some values obtained at high redshifts. Together with low metallicities this make Magellanic Clouds to be an interesting test case to study of the central parts of high redshift galaxies.

==> journals.tex <==
\def\apj{Astroph. J.}
\def\apjl{Astroph. J. Lett.}
\def\apjs{Astroph. J. Suppl.}
%\def\mnras{Mon. Not. Roy. Astron. Soc.}
\def\mnras{MNRAS}
\def\nat{Nature}
\def\aap{Astron. Astroph.}
\def\pr{Phys. Rev.}
\def\pra{Phys. Rev. {\rm A}}
\def\prc{Phys. Rev. {\rm C}}
\def\prb{Phys. Rev. {\rm B}}
\def\prd{Phys. Rev. {\rm D}}
\def\prl{Phys. Rev. Lett.}
\def\plb{Physics Letters {\rm B}}
\def\apss{Astroph. Space Sci.}
\def\pla{Physics Letters {\rm A}}
\def\ssr{Space Sci. Rev.}
\def\araa{Ann. Rev. Astron. Astroph.}
\def\aj{Astron. J.}
\def\pasp{Pub. Astron. Soc. Pacific}
